Navigating the landscape of multimodal AI in medicine: a scoping review on technical challenges and clinical applications

Recent technological advances in healthcare have led to unprecedented growth in patient data quantity and diversity. While artificial intelligence (AI) models have shown promising results in analyzing individual data modalities, there is increasing recognition that models integrating multiple complementary data sources, so-called multimodal AI, could enhance clinical decision-making. This scoping review examines the landscape of deep learning-based multimodal AI applications across the medical domain, analyzing 432 papers published between 2018 and 2024. We provide an extensive overview of multimodal AI development across different medical disciplines, examining various architectural approaches, fusion strategies, and common application areas. Our analysis reveals that multimodal AI models consistently outperform their unimodal counterparts, with an average improvement of 6.2 percentage points in AUC. However, several challenges persist, including cross-departmental coordination, heterogeneous data characteristics, and incomplete datasets. We critically assess the technical and practical challenges in developing multimodal AI systems and discuss potential strategies for their clinical implementation, including a brief overview of commercially available multimodal AI models for clinical decision-making. Additionally, we identify key factors driving multimodal AI development and propose recommendations to accelerate the field's maturation. This review provides researchers and clinicians with a thorough understanding of the current state, challenges, and future directions of multimodal AI in medicine.

==> deprecated_individual_sections/abbreviations.tex <==

This is just a nice overview for ourselves to keep track of abbreviations we may use. In the official MEDIA reviews these do not seem to be present. If you use any of these abbreviations in your text, please check whether it's appropriate to spell it out or use the abbreviation. If you introduce any new abbreviations, please add them to this (alphabetical!) list.

\begin{table}[htbp]
\centering
\caption{List of Abbreviations}
\label{tab:abbreviations}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Abbreviation} & \textbf{Full Form} & \textbf{First introduced} \\
\midrule
ADNI & Alzheimer’s Disease Neuroimaging Initiative & Overview \\
AI & Artificial Intelligence & Introduction \\
AUC & Area under the curve & Architecture choices \\
AUROC & Area under the receiver operating curve & Road to clinic \\
CE & Conformité Européenne & Road to clinic \\
CNN & Convolutional Neural Network & Introduction \\
DL & Deep Learning & Search \\
FDA & Food and Drug Administration & Road to clinic \\
MIMIC & Medical Information Mart for Intensive Care & Overview \\
MLP & Multi-layer perceptron & Overview \\
TiAb & Title Abstract & Search \\
TCGA & The Cancer Genome Atlas & Overview \\
TCIA & The Cancer Imaging Archive & Overview \\
OCT & Optical Coherence Tomography & Overview \\
RNN & Recurrent Neural Network & Overview \\
ViT & Vision Transformer & Overview \\
WSI & Whole slide image & Medical tasks \\
\bottomrule
\end{tabular}
\end{table}

==> deprecated_individual_sections/architecture_choices.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Architecture choices} \label{sssec:architecture choices}

%\subsubsection{Dataset handling and feature extraction}
%As mentioned earlier, the most common approach for multimodal analysis involves the usage of imaging (e.g., MRI, PET, histopathology WSIs) and a non-imaging modality (e.g., omics, medical reports, clinical information). This data then has to be processed in some way for fusion to take place. For example, radiology and pathology imaging data often undergo feature extraction and segmentation before it is fused with non-imaging data, like clinical information. Non-imaging modalities may require less processing as they are usually in a structured format already and could therefore be directly combined with extracted features of the imaging modalities, as has been done in papers such as \cite{krstev_multimodal_2022, keicher_multimodal_2023, verma_multimodal_2023, matsuo_prognosis_2023,zhao_multimodal_2022}. On the other hand, for many multimodal models using radiology, the data is first (pre-)processed through a feature extraction model - often a convolutional neural network [ref].

%Architecture choices such as fusion point (intermediate is the most prevalent, but late fusion is also common), fusion methods (concatenation and ensembling being the most important) and type of feature extraction used (machine learning, CNN, VAE, etc.) are the most important factors. Additionally, the model itself has to handle missing or incomplete data in certain ways, related to Daan's part - machine learning methods and e.g. ensembling can often handle this, but deep learning methods that use e.g. concatenation can't. Some interesting models include the Student-Teacher model, integrated learning approaches (especially those that fuse in an earlier stage) and those that can do multiple things at once.
%Small overview for myself:

%\begin{itemize}
%\item Distribution in fusion moments (early/inter/late)
%\item Dataset handling (feature extraction, feature vector creation, ensembling, etc.)
%\item Papers that tried multiple architectures and their results
%\item Papers that have unorthodox and highly effective architectures and fusion methods
%\item Best practices for when building a multimodal model
%\end{itemize}

%Aside from the timing at which data sources are merged, a crucial decision must be made regarding the method by which data is combined. Although this is inherently tied to the previous methods mentioned (for example, majority voting is practically exclusive to late fusion), there are cases in which data fusion methods may vary.

%For example, the vast majority of the models studied in this review [\textcolor{red}{around 200 papers, add some references}] concatenate clinical data directly with extracted features from their extracted imaging or omics features, \cite{ross_external_2024}. Lee et al. \cite{lee_predicting_2019} opted for concatenation-based data integration, stating that concatenation is conceptually the simplest method to integrate multiple data sources into a single vector. \ref{fig:fig_distribution_of_encoder_fusion_modality} contains an overview of the encoding techniques and their correlations with the fusion stages.

%Although this form of simple concatenation is the most common technique used for intermediate fusion, its effectiveness has also been challenged: for example, \cite{cahan_multimodal_2023} explicitly states that "the common practice is simple concatenation, but we believe this is not enough to utilize inter-modality correlations. The implementation of some form of dimensionality reduction, for example, principal component analysis (PCA), has been shown to improve the performance of multimodal fusion by helping the network learn associations between modalities due to distinct underlying distributions" (Yi, D., Lei, Z., Liao, S. and Li, S. Z. Shared representation learning for heterogeneous face recognition. arXiv:1406.1247 (2014).).". 

%There are also other, more advanced fusion methods, like attention learning [\textcolor{red}{references}], in which different data sources are integrated in a more step-wise manner. For late fusion, the three methods described earlier all appear in roughly equal proportions [\textcolor{red}{numbers + references}]. Lastly, for early fusion, the aforementioned attention learning often occurs with various bespoke methods, although the sample size is still small here.
%However, as the models started to become more complex over time, usually causing the fusion step to be earlier, various models that utilize unique ways of merging the data have been proposed. Some of these include:


The architecture choices for multimodal AI models often rely on the purpose(s) of the model and data availability. Regardless, the key steps taken when designing such a model include the same core functionalities in feature extraction, data fusion and final processing of the fused data. All of these steps can have many differences in their approaches, and although these steps have to be done in order, they can be done simultaneously. Some papers also introduce explainability \cite{ketabi_multimodal_2023, yang_deep_2021, parvin_convolutional_2024} into their models or attempt to construct multiple different model architectures to assess the effectiveness of each variant (e.g. \cite{huang_multimodal_2020, lopez_reducing_2020}). 

\subsubsection{Dataset handling and feature extraction}
As mentioned earlier, the most common approach for multimodal analysis involves the usage of an imaging (e.g. MRI, PET, histopathology WSIs) and a non-imaging modality (e.g. omics, medical reports, clinical information). This data then has to be processed in some way in order for fusion to take place. For example, radiology and pathology imaging data often undergoes feature extraction and segmentation before it is being fused with non-imaging data, like clinical information. Non-imaging modalities may require less processing as they are usually in a structured format already and could therefore be directly combined with extracted features of the imaging modalities, as has been done in papers such as \cite{krstev_multimodal_2022, keicher_multimodal_2023, verma_multimodal_2023, matsuo_prognosis_2023,zhao_multimodal_2022}. On the other hand, for many multimodal models using radiology, the data is first (pre-)processed through a feature extraction model - often a convolutional neural network [ref].

\subsubsection{Feature fusion}
A key feature of multimodal data is the method in which each data source is linked to each other. This can vary in both the way in which the data itself is merged, but is also influenced by the model structure, which may dictate at which point information from different data sources is combined.
Out of all papers reviewed in this study, the vast majority \textcolor{red}{(79\%, 243/308 papers)} utilized intermediate fusion (alternatively called "joint" \cite{huang2020fusion} or "multiscale" fusion), in which data sources get fused after feature extraction, but before the final decision making. Considering the majority of the papers also incorporate tabular data (e.g. through omics or clinical variables) \textcolor{red}{(77\%)} with features extracted from imaging data, a solution often used is to concatenate the feature vectors of both modalities together before the combined set of features goes through a final decision model.

Late fusion, a method in where modality fusion is performed at the decision level, is the second most common technique \textcolor{red}{(15\%)}. These architectures can often look similar to those from intermediate fusion models, with the main difference being that no additional feature extraction steps are being taken after fusion outside of the final decision making process. Most of these papers extract features and subsequent decisions from separate unimodal networks, then algorithmically fuse the modalities together to get an \textit{overall} decision. This can be achieved by applying a (weighted) average over the results of each modality, through regression analysis and by ensembling a set of outcomes from the outcomes of the unimodal models. These models are the easiest to implement or to build on top of existing unimodal methods as some can be as simple as taking the average between modalities \citep{lopez_reducing_2020}, but since the model's context between each data modality is very restricted, they may also provide limited benefits. Some papers also mention "concatenation" is used for late fusion, but these often lead into statistical approaches, like regression methods, or simple machine learning approaches like support vector machines and random forests.

The last method involves early fusion, at which modalities are fused at the data imputation level: there is at most some pre-processing involved, but no feature extraction takes place prior to data fusion. Our study found that this fusion method has so far been applied the least: \textcolor{red}{6\%} of the papers included in this study have used some form of early fusion. The majority of these papers (61\%, 14/23) were also released in 2023 or later, as fusing different data sources early is difficult to transfer between different data types and could therefore require a bespoke setup. A commonly used technique for early fusion is transfer (or attention) learning \textcolor{red}{(x\%, x/308 papers)}: a technique where a model learns from pattern representations with respect to each modality (including itself) \textcolor{red}{references}. 

One of the main reasons why intermediate and late fusion are more abundant is due to their relative simplicity in implementation and compatibility with existing (unimodal) models and datasets. A popular example involves the ADNI dataset for Alzheimer's and Mild Cognitive Impairment (MCI), where features extracted from both the imaging and clinical data are commonly used for intermediate or late fusion. Since extensive feature extraction algorithms exist for both the radiology and clinical datasets, the only required additions involve the desired fusion approach (often through concatenation or regression [add percentages]) and a final convolutional layer to extract the model's final decision \cite{mostapha_braided_2020, liu_cascaded_2023, yang_deep_2021, mirabnahrazam_predicting_2023, pena_toward_2022}.

\onecolumn
\begin{figure}%
    \centering
    \includegraphics[width=15cm]{figures/Multimodal AI Overview V5.png}%
    \caption{Figure 6: a simplified 
    schematic view of the different fusion stages. \textcolor{red}{(And types?)}}% 
    \label{fig:Multimodal_Fusion}%
\end{figure}


\twocolumn

Aside from the timing at which data sources are merged, there is also an important decision to be made with the method in which data is combined. Although this is inherently tied to the previous methods mentioned (for example, majority voting is practically exclusive to late fusion), there are cases in which data fusion methods may vary. For example, the vast majority of the models studied in this review [\textcolor{red}{around 200 papers, add some references}] simply concatenate clinical data directly with extracted features from their extracted imaging or omics features, for example \cite{ross_external_2024}. In fact, Lee et al. \cite{lee_predicting_2019} opted for concatenation-based data integration, stating that concatenation is conceptually the simplest method to integrate multiple sources of data into a single vector. Figure 4 contains an overview of the encoding methods used and their correlations with the fusion stages. \newline
Although this form of simple concatenation is the most common technique used for intermediate fusion, its effectiveness has also been challenged: for example, \cite{cahan_multimodal_2023} explicitly states that "the common practice is simple concatenation, but we believe this is not enough to utilize inter-modality correlations. The implementation of some form of dimensionality reduction; for example, principal component analysis (PCA), has been shown to improve performance of multimodal  fusion by helping the network learn associations between modalities due to distinct underlying distributions" (Yi, D., Lei, Z., Liao, S. and Li, S. Z. Shared representation learning for heterogeneous face recognition. arXiv:1406.1247 (2014).).". 

There are also other, more advanced fusion methods, like attention learning [\textcolor{red}{references}], in which different data sources are integrated in a more step-wise manner. For late fusion, the three methods described earlier all appear in roughly equal proportions [\textcolor{red}{numbers + references}]. Lastly, for early fusion, the aforementioned attention learning often appears here, together with a variety of bespoke methods, although the sample size is still small here.
However, as the models started to become more complex over time, usually causing the fusion step to be earlier, a variety of models have been proposed that utilize unique ways of merging the data. Some of these include:

\begin{itemize}
    \item Mallya and Hamarneh \cite{mallya_deep_2022} utilize a \textit{student-teacher model}, in which the knowledge learned from one model (and by extension, modality) is transferred to another, optimizing the performance at the training level and then allow for unimodal inference when testing the model;
    \item Wang et al. \cite{wang_predicting_2023} and Yang et al. \cite{yang_prediction_2022} applies data fusion through \textit{compact bilinear pooling} and \textit{Multimodal Compact Bilinear Pooling}, respectively, which uses a linear kernel machine to reduce the dimensions of the fused features;
    \item Antoher paper by Wang et al. \cite{wang_multi-modality_2024}, uses \textit{Multimodal Factorized Bilinear Pooling}, another sophisticated feature fusion technique that outperformed simple concatenation (0.73 C-index vs. 0.68);
    \item Ren et al. \cite{ren_deep_2021} apply the fusion in Fourier space, then apply the inverse transform before processing the data through another neural network;
    \item Pelka et al. \cite{pelka_sociodemographic_2020} uses a "branding marker" to add white bars on unused areas of an MRI image, directly encoding and fusing the metadata onto the MRI image to then be used for training;
    \item Li and Ogino \cite{li_augmented_2020} use an advanced transfer learning system (called "augmented radiology" by the authors) in which features are directly interchanged between radiological and pathological images;
    \item Mostapha et al. \cite{mostapha_braided_2020} apply a \textit{braided U-net}, which utilizes multiple convolutional networks to introduce both a unimodal dataset (e.g. image data) and a combined set (in this case with patient metadata) to fuse the datasets at an early stage;
    \item Lastly, Zhang et al. \cite{zhang_text-guided_2023} apply a \textit{foundation model} to extend a text embedding model towards classifying pathological images.
\end{itemize}

\subsubsection{Assessment and effectiveness of multimodal approaches}
Aside from attempting to innovate on multimodal AI for medical imaging, one must also assess whether these methods actually surpass their corresponding unimodal approaches. In general, multimodal approaches perform consistently better than unimodal approaches, although the levels of improvement can vary. \cite{schilcher_fusion_2024} reports an improvement on the AUC of about 0.02 (0.97 over 0.95), whereas Yin et al. \cite{yin_development_2024} report an improvement with an AUC improvement from 0.749 (at best) to 0.916. The additional data provided in these multimodal approaches can cause an improvement in accuracy and may be easy to implement, but the improvement in terms of scoring metrics vary wildly. For example, some papers tried both a unimodal (only imaging) and multimodal (imaging and tabular data, like clinical variables or omics) approach \cite{samak_prediction_2020, vale-silva_long-term_2021, pei_hybrid_2021}, but only see an improvement of less than 5\% (relative to the baseline) for the AUC or accuracy for the multimodal approach. On the other hand, a model by Kim and Shin \cite{kim_prediction_2023} shows that the addition of tabular clinical data can also cause a key improvement in diagnosis or survival analysis. The feature extraction is often done independently and the way in which a model handles data also has an impact in the case when data is missing (see \textcolor{red}{(section 3.2.1)}). A more interesting part of these comparisons, however, are the ablation studies - although only some studies have included these, the ones who do give a good insight in the robustness of the model \cite{xie_deep_2022, plotka_babynet_2023, liu_cascaded_2023, zheng_graph_2024, cahan_multimodal_2023}. This is especially important for multimodal models as data is often incomplete or has to be filled by other means (see \textcolor{red}{section 3.2.1}). This has also lead to some interesting results: for example, \cite{sahasrabudhe_deep_2021} showed that the improvements with the clinical data only marginally improved their model. Ablation studies and comparisons with earlier models (regardless of whether they are unimodal or multimodal) could therefore give valuable insights on how and when a multimodal model should be developed.


%Architecture choices such as fusion point (intermediate is the most prevalent, but late fusion is also common), fusion methods (concatenation and ensembling being the most important) and type of feature extraction used (machine learning, CNN, VAE, etc.) are the most important factors. Additionally, the model itself has to handle missing or incomplete data in certain ways, related to Daan's part - machine learning methods and e.g. ensembling can often handle this, but deep learning methods that use e.g. concatenation can't. Some interesting models include the Student-Teacher model, integrated learning approaches (especially those that fuse in an earlier stage) and those that can do multiple things at once.
%Small overview for myself:

%\begin{itemize}
%\item Distribution in fusion moments (early/inter/late)
%\item Dataset handling (feature extraction, feature vector creation, ensembling, etc.)
%\item Papers that tried multiple architectures and their results
%\item Papers that have unorthodox and highly effective architectures and fusion methods
%\item Best practices for when building a multimodal model
%\end{itemize}

==> deprecated_individual_sections/clinical_applications.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Clinical applications} 
\label{sssec:Clinical applications}
Subdiving multimodal AI research papers based on the applied organ system reveals significant variations in the development of multimodal models. The majority of studies have concentrated on the nervous system (n=125), followed by the respiratory system (n=93), digestive (n=43) and reproductive (n=43) systems, sensory system (n=26), integumentary system (n=24), and the cardiovascular system (n=20). Fewer studies have been published in musculoskeletal (n=11) and urinary (n=12) systems. Some studies evaluated their models into more than one system and, therefore, are reported in a separate \textit{Multiple Systems} category (n=24). Papers that did not align with any of these categories were grouped into a \textit{Miscellaneous} category (n=15). Below, we summarize the key contributions in each area.

\textbf{Nervous system (n=125)}\\
The predominant focus on the nervous system has been on diagnosis and prognosis disease progression of neurodegenerative disorders, such as Alzheimer's disease and mild cognitive impairment (n=46), with a few studies focusing on Parkinson's disease (n=9) and dementia (n=2). The second major focus is on cancer diagnosis and survival prediction (n=22). Other studies focused on the diagnosis of autism (n=6), stroke (n=7), and mental disorders, such as schizophrenia (n=6) and depression (n=4). The analyses of these papers showed that most studies in this area utilize MRI as the primary modality, integrating either clinical data (n=44) or omics data (n=18) for a multimodal approach, or all three for the same task (n=8). Other studies combined pathology with MRI images (n=6) or omics (5), and CT with clinical variables (n=10).  
A significant number of studies utilized publicly available datasets (n=102), with Alzheimer’s Disease Neuroimaging Initiative (ADNI) dataset being the most frequently used (n=45), followed by The Cancer Genome Atlas (TCGA)(n=11), Computational Precision Medicine Radiology-Pathology challenge on brain tumor classification dataset (CPM-RadPath) (n=6) and Brain Tumor Segmentation Challenge (BraTS) (n=3). Only a limited number of studies conducted external validation of their models (n=15), while the majority employed cross-validation (n=64) and internal validation (n=40). The integration of multiple modalities has been shown to enhance performance in most of these studies (n=86), underscoring the value of incorporating additional data sources that capture information not evident in a single modality alone.

Some studies stood out for their system design and development. 
Some of these focused on glioma grading, such as \citet{li_augmented_2020} that proposed a patient-wise feature transfer model that learns the relationship between radiological and pathological images, and \citet{cui_multi-modal_2022} that integrated histological images and genomic data utilizing all available data from patients with both complete and partial modalities. \citet{cui_survival_2022} present a multimodal learning pipeline based on radiology, pathology, genomic, and demographic data for handling missing data reaching competitive performance on glioma tumor survival prediction.
Several interesting studies focused on Alzheimer's prediction, such as \citet{liu_cascaded_2023} that employed multiple transformer architectures to integrate imaging data and clinical variables demonstrating robustness even in scenarios with missing data, and \citet{xu_multi-modal_2022} combined latent representations, imputation modules, and a recurrent neural network (RNN) to handle variable inputs from MRI, PET, and clinical variables for modeling Alzheimer's progression. \citet{pelka_sociodemographic_2020} diagnosed early and subclinical stages of Alzheimer’s Disease using sociodemographic data with MRI scans. \citet{lei_alzheimers_2024} developed a novel framework for AD diagnosis that fuses gene, imaging, protein, and clinical data, validating the proposed method on the ADNI dataset and outperforming other state-of-the-art multimodal fusion methods. 
Other interesting examples are the one of \citet{kim_multimodal_2024} that predicted Parkinson’s disease (PD) progression integrating diverse biomarkers from structured clinical assessments, imaging data, and biospecimen information, and the study of \citet{xue_ai-based_2024} that presented an AI model that integrates diverse data, including clinical data, functional evaluations, and multimodal neuroimaging, to identify 10 distinct dementia etiologies across 51,269 participants from 9 independent datasets, even in the presence of incomplete data.

\textbf{Respiratory system (n=93)}\\
Research in the respiratory system predominantly focused on diagnosis (n=10), survival (n=9), treatment prediction (n=3), and progression (n=2) of cancer, and on diagnosis (n=20), survival (n=3) and disease progression (n=2) of Covid-19. Across these studies, the common strategy involves combining clinical variables with either X-ray or CT imaging of the thorax (n=18 and n=27, respectively). Additionally, a subset of papers (n=11) developed vision-language models by integrating chest X-rays with clinical reports, specifically for X-ray report generation. The majority of the studies regarding respiratory diseases employed public datasets, such as the MIMIC-CXR dataset (n=12), The Cancer Genome Atlas (TCGA) (n=4), and the Radiological Society of North America (RSNA) dataset (n=2). Two notable observations in this anatomical subset relate to the comparatively high proportion of studies (n=15) employing external validation and to the high number of studies that obtained higher performances when performing multimodal integration than using single-modality models (n=68). 

Among the most interesting studies of the respiratory category, \citet{lee_development_2022} utilized a commercially available chest X-ray abnormality detection model to extract features, which were then integrated with clinical variables and laboratory findings to predict prognostic and intervention outcomes in COVID-19 patients. \citet{keicher_multimodal_2023} proposed a multimodal graph‑based approach combining imaging and non‑imaging information to predict COVID-19 patient outcomes, namely intensive care unite admission, need for ventilation, and mortality. 
\citet{gao_reducing_2022} proposed a multimodal approach combining CT imaging and clinical variables to enhance cancer risk estimation in patients with indeterminate pulmonary nodules. 
\citet{gao_deep_2021} proposed multi-path multi-modal missing network (M3Net), a system integrating multimodal data, including clinical data, biomarkers, and CT images, that can be trained end-to-end with all data types or make predictions using a single modality. Cross-validation and external validation showed that combining multiple modalities significantly improves performances in predicting lung cancer risk compared to using a single modality. 
\citet{wang_multi-modality_2024} proposed a novel framework for lung cancer survival analysis snd introducing a multi-modality fusion module and multi-task learning based on histopathology images and clinical information.
\citet{kumar_deep-learning-enabled_2023} combined X-ray with clinical information to develop a multimodal fusion approach to detect lung disease and developed two architectures of multimodal network based on late and intermediate fusion, showing better performances with the latter. 
\citet{lopez_reducing_2020} examined deep learning-based multimodal fusion techniques for the classification of several chest diseases using radiological images and associated text reports. 


\textbf{Digestive system (n=43)}\\
In the domain of the digestive system, most studies focused on the diagnosis of malignancies (n=25), with fewer addressing survival (n=10), treatment response (n=3) and disease progression prediction (n=2). The primary malignancies investigated include colorectal (n=13) and liver (n=10) cancers, with some studies also focusing on the stomach, esophagus, and duodenum (n=8). Similar to the scenario with reproductive system studies, no single modality combination was dominant in this field, though clinical variables (n=29) and histopathology slides (n=16) were commonly included. The integration of multimodal data improved performance in 38/39 papers when compared to unimodal approaches. However, external validation was relatively uncommon (n=11), proposing the need for a greater availability of public datasets. Indeed, not a high percentage of the studies employed publicly available datasets (n=17), including mainly TCGA (n=11). 

Several studies were particularly noteworthy. \citet{cui_diagnosing_2024} developed a multimodal AI model, using both endoscopic ultrasonography images and clinical information to distinguish carcinoma from noncancerous lesions, tested this model in internal, external, and prospective datasets, and evaluated the assisting potential of the model in a crossover trial. Their results showed that AI assistance significantly improved the diagnostic accuracy of novice endoscopists and that the additional interpretability information helped reduce skepticism among experienced endoscopists.
\citet{chen_predicting_2024} introduced the Multi-Modal model (MuMo), a deep learning model combining radiology, pathology, and clinical information to predict treatment responses to anti-HER2 therapy or anti-HER2 combined immunotherapy in patients with HER2-positive gastric cancer. 
\citet{guo_prediction_2023} proposed a multi-scale multiple instance learning approach to extract information from histopathology slides and integrate it with clinical variables for predicting lymph node metastasis in primary gastric cancer. \citet{zhou_integrative_2023} combined histopathology slides, clinical variables, and mutation signatures for patient stratification in colon adenocarcinoma. \citet{zhou_deep_2023} merged PET/CT features, histopathology slides, and clinical data to predict treatment response to bevacizumab in liver metastasis originating from colorectal cancer.


\textbf{Reproductive system (n=43)}\\
The reproductive domain encompasses studies focused on the diagnosis and prognosis prediction of malignancies mainly in breast (n=33), followed by the prostate (n=5), ovaries, cervix and placenta (n=5).  Unlike other domains, there was no predominant combination of modalities; clinical variables with MRI (n=9) or histopathology (n=6), omics data with histopathology (n=5) or clinical data (n=3) were explored with similar frequency. The use of external validation was found only in a few studies (n=9). Some studies employed public datasets, such as the TCGA-BRCA dataset (n=11).

Among interesting studies, \citet{esteva_prostate_2022} developed a multimodal deep learning architecture trained on clinical data and digital histopathology from prostate biopsies to predict long-term outcomes of prostate cancer patients. They validated their models using five phase III randomized trials conducted across hundreds of clinical centers and obtained discriminatory performances superior to the most common risk-stratification tools. \citet{priester_prediction_2023} combined MRI, prostate-specific antigen values, and prostate biopsy results to detect prostate cancer. 
Some interesting studies focused on breast diseases, such as \citet{mondol_biofusionnet_2024} presented BioFusionNet, a deep learning framework that fuses image-derived features with genetic and clinical data and that outperformed state-of-the-art methods in performing survival risk stratification of ER+ breast cancer patients.
\citet{holste_end--end_2021} evaluated various methods for fusing MRI and clinical variables in breast cancer classification. \citet{wang_predicting_2023} explored multiple instance learning techniques to combine histopathology with clinical features to predict the prognosis of HER2-positive breast cancer patients. \citet{joo_multimodal_2021} integrated imaging features from both T1- and T2-weighted MRI along with clinical features to predict treatment response to neoadjuvant chemotherapy in breast cancer. Regarding renal diseases, \citet{ning_integrative_2020} developed a comprehensive fusion method that integrated RNA sequencing, CT imaging, histopathology, and clinical variables for prognosis prediction in clear cell renal cell carcinoma. 

\textbf{Sensory system (n=26)}\\
In the sensory system, the majority of multimodal models have focused on ophthalmology (n=24), with the remaining studies addressing otology (n=2). Within ophthalmology, there is a distinct focus on glaucoma (n=7), followed by retinopathy (n=4). Three modalities are the most used in these studies: optical coherence tomography, color fundus photography, and clinical data, in different combinations. However, only a small number of papers included external validation (n=3) or used publicly available datasets (n=10).

This category included several interesting studies in the ophtalmology field. For example \citet{nderitu_predicting_2024} developed a deep learning system to predict 1, 2, and 3 year progression of diabetic retinopathy using risk factor characteristics and colour fundal images. \citet{mehta_automated_2021} integrated optical coherence tomography, color fundus photography, and clinical variables to diagnose glaucoma. 
\citet{zhou_uncertainty-aware_2024} employed a multimodal approach that combined four imaging modalities with free-text lesion descriptions for uncertainty-aware classification of retinal artery occlusion. Regarding otology, \citet{sundgaard_multimodal_2024} followed an unconventional multimodal approach by integrating wideband tympanometry (a signal) with otoscopy (an image) to demonstrate that disparate data types can be effectively fused with the appropriate model architecture. 

\textbf{Integumentary system (n=24)}\\
All studies within the integumentary category focused on the diagnosis of skin lesions, primarily through the fusion of dermatoscopic images and clinical variables (n=12). The majority of the studies (n=14) compared multimodal approaches to unimodal baselines and reported improved performance with the addition of extra modalities, suggesting that factors such as lesion location and patient demographics contribute valuable information. Notably, one paper conducted prospective validation of its findings \citep{zhu_deep_2024}. Among the remaining studies, only four carried out external validation, while all others relied on internal validation or cross-validation approaches. In contrast to other systems, several publicly available datasets are readily accessible. The most used one is the dataset coming from the ISIC challenge (n=8), followed by HAM10000 (n=4), Seven-point Criteria Evaluation (SPC) (n=2). Other public datasets in this category include Gland Segmentation in Colon Histology Images Challenge (GlaS), PAD-UFES-20 datasets, and TCGA.

Worth mentioning, among the most interesting examples of this category, \citet{zhou_pre-trained_2024} presented SkinGPT-4, an interactive dermatology diagnostic system based on multimodal large language models and trained on pairs of images and textual descriptions. SkinGPT-4 was evaluated on 150 real-life cases in collaboration with board-certified dermatologists. This system allows users to upload their own skin photographs for diagnosis, enabling it to autonomously assess the images, identify the characteristics and classifications of skin conditions, conduct in-depth analyses, and offer interactive treatment recommendations. Other interesting studies includes \citet{tang_fusionm4net_2022} that proposed two fusion schemes to efficiently integrate dermatoscopic images, clinical photographs and clinical variables for the diagnosis of eight types of skin lesions, and \citet{zhu_deep_2024} that demonstrated that their multimodal model, which incorporated clinical images and high-frequency ultrasound, performed on par or better than dermatologists in diagnosing seventeen different skin diseases. 

\textbf{Cardiovascular (n=20)}\\
Research in the cardiovascular domain was exclusively focused on the diagnosis of heart diseases (n=15), with some studies focusing also on survival, treatment response and disease progression prediction (n=4). In all but two studies, the proposed models incorporated clinical variables with a second modality, often in conjunction with radiology imaging (n=7). When comparing the multimodal models to the unimodal ones, most of the studies obtained better results with the latter (n=14). However, also in this case, only three studies externally validated their results. Interestingly, some publicly available datasets were employed, including MIMIC, JSRT Database, Montgomery County X-ray Set, and data coming from the Gene Expression Omnibus (GEO) and UK Biobank. 

An interesting example in this category is the study of \citet{v_novel_2024} that introduced an Attention-Based Cross-Modal (ABCM) transfer learning framework to predict cardiovascular disease merging diverse data types, including clinical records, medical imaging, and genetic information, through an attention-driven mechanism.


\textbf{Urinary system (n=11)}\\
In the urogenital system, the majority of studies focused on the diagnosis of kidney (n=7) disorders, with fewer addressing bladder (n=2) and adrenal gland (n=1) conditions. These multimodal studies were employed for diagnosis (n=8) or survival prediction (n=4) predominantly on oncological malignancies (n=9) with fewer on renal artery stenosis, chronic kidney disease, and one aiming at performing report generation. Most of the studies employed CT images combined with a second modality (n=9), such as clinical data, histopathology images, and omics. Most studies (n=8) demonstrated improved performance with multimodal models compared to unimodal ones. Similarly to other systems, only a small number (2/11) externally validated their results, while the majority used either internal validation or cross-validation approaches. A few public datasets are available for this category: The Cancer Genome Atlas (TCGA) and The Cancer Imaging Archive (TCIA).  
An interesting study focusing on renal diseases proposed a cross-modal feature-based integrative system combining computed tomography, histopathological images, and genomic data, to construct a prognostic model for clear cell renal cell carcinoma \citep{ning_integrative_2020}.

\textbf{Musculoskeletal system (n=11)}\\
In the musculoskeletal system, studies focused on the diagnosis of bone (n=6) diseases, with fewer addressing teeth and muscle conditions, focusing on the diagnosis of pathological gait, osteoarthritis, deep caries and pulpitis, bone fractures and aging, and soft tissue sarcoma. These studies mostly employed radiology images together with clinical data (n=6) or unstructured text data (n=2). Most studies (n=8) demonstrated improved performance with multimodal models compared to unimodal ones. However, no studies externally validated their results, mainly employing internal validation approaches. Two public datasets were employed in this category, coming from the Osteoarthritis Initiative (OAI) and the Pediatric Bone Age Challenge. 
An interesting study of \textit{Schilcher et al.} aggregated X-ray imaging and clinical information from 72 radiology departments in Sweden to develop a multimodal model for detecting atypical femur fractures \cite{schilcher_fusion_2024}.

\textbf{Multiple systems (n=24)}
This category includes papers that interestingly evaluated the multimodal system on multiple organs belonging to different systems. An aspect worth mentioning is that all these studies benefited from available public datasets, confirming that the presence of publicly available data is particularly important for the development and assessment of multimodal AI systems. The majority of the studies in this category evaluated the performance of their models across diseases affecting up to five different organs (n=20). Four studies were distinguished by the extensive range of organs on which they assessed their models: 
\cite{azher_assessment_2023} developed an interpretable multimodal modeling framework that combines DNA methylation, gene expression, and histopathology for prognostication of eight types of cancers;
\cite{chen_pan-cancer_2022} developed a multimodal deep learning model to jointly examine pathology whole slide images and molecular profile data from 14 cancer types to predict outcomes and discover prognostic features that correlate with poor and favorable outcomes, Notably, their method incorporated a strong explainability component with heatmaps for histopathology and SHAP values for genomic markers, serving as justification for the predicted risk stratification;
\cite{cheerla_deep_2019} constructed a multimodal neural network-based model to predict the survival of patients for 20 different cancer types using clinical data, mRNA expression data, microRNA expression data, and histopathology whole slide images (WSIs); 
\cite{vale-silva_long-term_2021} presented MultiSurv, a multimodal deep learning method for longterm pan‑cancer survival prediction that was applied to data from 33 different cancer types. These four studies demonstrated the reliability of their models on a wide range of cancer types to do that, interestingly, all four benefited from the publicly available data of TCGA.
Other interesting studies are:
"ContIG: Self-supervised Multimodal Contrastive Learning for Medical Imaging with Genetics" propose ContIG, a self-supervised method that integrates medical images and genetic data and uncovers novel relationships through genome-wide association studies. For Diabetic Retinopathy detection, predict cardiovascular risk factors, and Pathological Myopia Segmentation.


\textbf{Miscellaneous (n=15)}\\
This category includes papers that do not fit into the aforementioned categories but provide novel or unique contributions to multimodal model development. Some interesting examples include \citet{kim_prediction_2023} that proposed a model employing an autoencoder with multiple encoders to extract comprehensive features from hormonal and pathological data and demonstrated that the proposed model significantly improves performance when compared to unimodal models when predicting the Recurrence Probability of Thyroid Cancer Patients. \citet{lee_prediction_2024} explored unsupervised learning by combining histopathology and clinical data, followed by knowledge distillation to derive an unimodal histopathology model for predicting immunochemotherapy response. 
\citet{khader_multimodal_2023} developed a transformer-based neural network architecture that integrates multimodal patient data, including both imaging and non-imaging, to diagnose up to 25 pathologic conditions and showed that the multimodal model significantly improves diagnostic accuracy when using both chest radiographs and clinical parameters compared to imaging alone and clinical data alone. Finally, \citet{cai_pre-trained_2023} presented VB-MVQA, a pre-trained multilevel fusion network that combines Vision-conditioned reasoning and Bilinear attentions to enhance feature extraction from medical images and questions. By incorporating Contrastive Language-Image Pre-training (CLIP) and stacked attention layers, VB-MVQA reduces language bias and improves accuracy. Experiments on three benchmark datasets showed that the proposed model surpasses state-of-the-art models.

REMINDER TO ADD THIS PAPER TO MAIN.TEX:
"ContIG: Self-supervised Multimodal Contrastive Learning for Medical Imaging with Genetics" propose ContIG, a self-supervised method that integrates medical images and genetic data and uncovers novel relationships through genome-wide association studies. For Diabetic Retinopathy detection, predict cardiovascular risk factors, and Pathological Myopia Segmentation.

==> deprecated_individual_sections/discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussion}

The exponential growth in multimodal AI models highlights the recent research efforts of multimodal data integration in healthcare. Although multimodal AI development poses unique challenges, the increasing research output in the field will inevitably lead to overcoming some of these challenges. Importantly, in line with a previous review \cite{kline_multimodal_2022}, our review revealed that integrating multiple data modalities leads to notable performance boosts. In the remainder of this section, we will highlight key takeaways of our analysis and provide recommendations for future research directions. 

The general state of the field of multimodal medical AI development was summarized in section \ref{overview_modalities}. This overview revealed significant disparities in multimodal AI development across various medical disciplines, tasks and data domains. Notably, multimodal AI development commonly found applications in the nervous system and the respiratory system. Conversely, applications in the musculoskeletal system or urinary system were scarce. Similar disparities are evident in the realm of data modality combinations. The integration of radiology imaging data and text data greatly outnumbered other combinations and was investigated in almost half of all papers in this review. On the other hand, integration of radiology and pathology data into multimodal frameworks seems to present greater challenges. Furthermore, substantial variations were observed in the model's application for a given medical task. The vast majority of models were aimed at automated diagnosis, whereas prediction of disease progression or survival was less common. 

Irrespective of the specific medical discipline or application, these discrepancies consistently point to a common factor: the availability (or lack thereof) of high-quality public datasets. The increased complexity associated with curating multimodal datasets, often requiring data collection from diverse sources (e.g. electronic health records or physical pathology slides) and departments (e.g. radiology and pathology), currently presents a significant bottleneck in model development. This challenge, however, also presents an opportunity for researchers and clinicians to make impactful contributions to the field, as the establishment of new multimodal datasets has the potential to substantially accelerate AI development in a certain domain. For instance, the publicly available ADNI (Alzheimer's Disease Neuroimaging Initiative) dataset has facilitated the development of more models for Alzheimer's diagnosis (n=n) than all studies combined in the musculoskeletal and urinary system. Apart from enabling domain-specific models, these public datasets can also stimulate research tackling general challenges associated with multimodal AI development. When datasets encompass as many as four distinct modalities (i.e. CT imaging, pathology slides, genomic data and text data), as seen in the TCGA-GBM dataset (The Cancer Genome Atlas Glioblastoma Multiforme Collection), this allows extensive investigations on the effects of missing data, model uncertainty, and model explainability with various data modalities. Hence, we believe that a community effort towards multimodal dataset development can have a strong propelling effect on the progress of the field. 
The technical design choices associated with processing and fusing data from diverse modalities were covered in sections \ref{sssec:Missing data handling} and \ref{sssec:architecture choices}. Our analysis revealed that the majority of studies prioritize the development of effective modality fusion methods over designing novel encoder architectures for optimal processing of different modalities. This was primarily evidenced by the comparatively large proportion of studies employing pretrained encoders for feature extraction from different modalities, after which the main contribution consisted of a novel, generally intermediate-level, fusion method. We posit that this observed focus on fusion methods rather than data encoders stems from the nature of multimodal datasets, which are typically smaller in scale compared to their unimodal counterparts. By leveraging encoders pre-trained on large unimodal datasets, and occasionally fine-tuning them on the available multimodal data, researchers can achieve robust performance despite the relative scarcity of multimodal data. Moreover, the great diversity of modalities in the medical field with their respective intricacies seems to warrant thorough investigation on optimal data fusion methodologies. Especially in light of the potential absence of certain modalities during inference, a robust fusion method is critical for reliable model predictions. The emergence of (medical) foundational models \cite{moor_foundation_2023}, which are generally multimodal, is expected to further accelerate research in optimal data fusion. Since these foundational models can further improve the availability of strong pre-trained encoders, this may further shift the research focus to designing optimal feature fusion methods.
The clinical applicability of current multimodal AI models, as discussed in subsection \ref{ssec:road_to_the_clinic}, reveals that the readiness of these models for clinical implementation lags behind that of unimodal models. We believe that this is influenced by the same challenges present in commercializing unimodal AI models, but amplified by the multimodal nature of these models. Although unimodal models require strong, preferably external, validation before deployment, this is even more prudent for multimodal AI models. Since multimodal models essentially consume larger amounts of data during deployment, there may be a greater risk for model drift when the distribution of one of the data modalities changes. Although extensive validation can investigate the effect of slight modality changes, such as using a slightly different staining in a multimodal model incorporating histopathology imaging data, this may lead to a combinatorial explosion when fusing an increasing amount of data modalities. A more optimistic foreseeable future could be that the presence of multiple modalities can serve a stabilizing purpose, where a noisy additional modality is unlikely to adversely influence the final prediction. However, we note that fusion of more than two modalities was encountered in only \textcolor{red}{placeholder!!}/\textcolor{red}{placeholder!!}(\textcolor{red}{placeholder!!}\%) papers, indicating that more evidence is needed to corroborate or disprove any of the aforementioned scenarios. Another amplified challenge in commercializing multimodal AI models is the call for explainable AI. Although this is already challenging for unimodal models, explainability in multimodal AI models likely requires explainability for each individual component (i.e. Shapley values for tabular data), but perhaps more importantly some degree of explainability how information from different sources is combined. Such an explainable multimodal AI model may also be able to alleviate the aforementioned risk of performance degradation under data drift for one of the data modalities. Given these challenges, we believe that the development of public multimodal datasets, preferably incorporating more than two modalities, will be an important stepping stone for advancing the field.

\section{Conclusion}
In conclusion, this review provides one of the most comprehensive overviews of multimodal AI development to date, spanning a wide range of medical disciplines, tasks and data domains. Although there is substantial evidence that multimodal AI models will incur significant performance boosts by taking a broader view of the patient, their development poses novel challenges. We hope that this review elucidated some of these challenges, but more importantly potential solutions, to guide the field in the years to come. 

==> deprecated_individual_sections/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}

The healthcare landscape is evolving rapidly, driven by an increasingly data-centric approach to patient care and decision-making \citep{shilo_axes_2020}. This shift is complemented by the advent of technologies such as digital pathology \citep{niazi_digital_2019}, biosensors \citep{sempionatto_wearable_2022}, and next-generation sequencing \citep{steyaert_multimodal_review_2023}, which provide clinicians with novel insights in various domains. The data generated by these diverse modalities is generally complementary, with each modality contributing unique information to the status of a patient. Some modalities offer a comprehensive overview at the macro level, while others may provide detailed information at single-cell resolution \citep{steyaert_multimodal_review_2023}. In addition to this recent growth in data quantity, there is a concurrent increase in the quality and diversity of available treatment options. Hence, selecting the optimal treatment has become increasingly complex, and a further data-centric approach to treatment selection may be required.  

The traditional approach to integrating information from different data modalities into a single decision is represented by multidisciplinary boards, where each specialized clinician offers their perspective on a given modality or piece of information in pursuit of consensus \citep{mano_implementing_2022}. Although establishing these boards has improved disease assessments and patient management plans \citep{mano_implementing_2022}, there is a foreseeable limit to the scalability of these boards. If data quantity and diversity continue to rise, many domain experts will be required to integrate these different information streams effectively. Fortunately, another technological advancement that is gaining a foothold in healthcare is artificial intelligence (AI). Although the vast majority of published work focuses on single modality applications of AI, several authors have highlighted the potential of AI systems to combine multiple streams of information, so-called multimodal AI, for decision-making \citep{steyaert_multimodal_review_2023, acosta_multimodal_2022, lipkova_artificial_2022}. These multimodal AI models are trained to process different streams of multimodal data effectively, leverage the complementary nature of information, and make an informed prediction based on a broader context of the patient's status. A recent scoping review corroborated this competitive edge of multimodal AI models, indicating that these models obtained a 6.4\% mean improvement in AUC compared to their unimodal counterparts \citep{kline_multimodal_2022}. However, despite these promising results, studies investigating multimodal AI models are comparatively scarce, and the development of unimodal models remains the de facto standard.

This lagging development of multimodal AI models can be attributed to several challenges. First, a practical challenge can be found in the cross-departmental nature of multimodal AI development. As different data modalities may originate from various medical departments, consulting different medical domain experts will likely be required for effective data integration. In addition, medical departments may have varying experience in data storage, retrieval, and processing, limiting the possibilities of multimodal AI development. For example, if a radiology department has a fully digital workflow while the corresponding pathology department does not, this effectively prohibits multimodal AI endeavors where whole slide images should be combined with radiological imaging data. 

Regarding model development, different data modalities can have vastly different characteristics, such as dimensionality or color space, which generally requires different AI model architectures tailored towards those modalities. For example, convolutional neural networks (CNN) were initially proposed for structured data, such as 2D and 3D images, but don't work for unstructured data. Conversely, transformers are solid, flexible encoders for various data modalities. Still, whether a one-size-fits-all architecture can capture various medical data modalities effectively remains unclear. In practice, multimodal data integration is commonly achieved by fusing different (intermediate) model outputs. Training multiple domain-specific AI models (i.e. encoders) and efficiently integrating these in a single prediction poses a challenge unique to multimodal AI development. 

Another notable challenge lies in the inconsistent availability of all modalities for each patient within a multimodal dataset. Patients with different disease trajectories will have various available modalities, leading to partially incomplete datasets. This can substantially reduce the adequate training dataset size for AI models that require complete multimodal data to generate predictions. Moreover, these issues also translate to implementation. If modalities are missing, it may be unclear how this impacts the model's performance, from the perspective of fewer available data to base a decision on and the potential introduction of population selection bias \citep{acosta_multimodal_2022}. In short, developing multimodal AI models poses several novel challenges compared to unimodal AI development.

Nevertheless, recent years have shown an accelerated interest in multimodal AI development for medical tasks \citep{salvi_multi-modality_2024}. In this review, we comprehensively summarize the state-of-the-art in multimodal AI development for medical tasks and investigate to what extent multimodal data integration is living up to its purported benefits. Unlike previous reviews that have focused on specific diseases, prediction tasks, or modality combinations \citep{acosta_multimodal_2022, salvi_multi-modality_2024, KRONES2025102690}, our analysis encompasses the full spectrum of the medical domain. Specifically, our review aims to shed light on I) the progress of multimodal AI model development across different medical disciplines and tasks, II) the technical challenges inherent in multimodal AI development, including model architectures, fusion methods, and the handling of missing data, III) the foreseeable road to the clinic of multimodal AI models, addressing aspects such as regulatory approval and explainability, and IV) the factors driving multimodal AI development and potential strategies to promote further maturation of this field. Lastly, we will provide an outlook on future perspectives in multimodal AI development based on our careful analysis of \textcolor{red}{NNN} papers published over the past six years (2018 - 2024).

==> deprecated_individual_sections/medical_tasks.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Clinical applications} 
\label{sssec:Medical tasks}
A classification of papers based on their functional system reveals significant variations in the development of multimodal models across different medical domains. The majority of studies have concentrated on the brain (n=\textcolor{red}{NNN}), followed by the respiratory system (n=\textcolor{red}{NNN}), breast (n=\textcolor{red}{NNN}), and the gastrointestinal system (n=\textcolor{red}{NNN}). Fewer studies have been published in the fields of sensory systems (n=\textcolor{red}{NNN}), dermatology (n=\textcolor{red}{NNN}), and the urogenital system (n=\textcolor{red}{NNN}). Papers that did not align with any of these categories were grouped into a miscellaneous category (n=\textcolor{red}{NNN}). Below, we summarize the key contributions in each area.

\textbf{Nervous system (n=121)}\\
The predominant focus within brain-related studies has been on Alzheimer's disease diagnosis (n=\textcolor{red}{NNN}) and glioblastoma diagnosis or survival prediction (n=\textcolor{red}{NNN} and n=\textcolor{red}{NNN}, respectively). For instance, \textit{Liu et al.} employed multiple transformer architectures to integrate imaging data and clinical variables for Alzheimer's classification, demonstrating robustness even in scenarios with missing data \cite{liu_cascaded_2023}. Similarly, \textit{Xu et al.} combined latent representations, imputation modules, and a recurrent neural network (RNN) to handle variable inputs from MRI, PET, and clinical variables for modeling Alzheimer's progression \cite{xu_multi-modal_2022}. Most studies in this area utilize MRI as the primary modality, integrating either clinical data (n=\textcolor{red}{NNN}) or omics data (n=\textcolor{red}{NNN}) for a multimodal approach. The integration of these modalities has been shown to enhance performance in \textcolor{red}{NNN}/\textcolor{red}{NNN} studies, underscoring the value of incorporating additional data sources that capture information not evident in MRI alone. 
Lastly, there is work covering the diagnosis of Parkinson's disease (n=\textcolor{red}{NNN}), schizophrenia (n=\textcolor{red}{NNN}), epilepsy (n=\textcolor{red}{NNN}) and stroke (n=\textcolor{red}{NNN}). 
In the brain category, a significant number of studies utilized publicly available datasets (n=\textcolor{red}{NNN}), with Alzheimer’s Disease Neuroimaging Initiative (ADNI) dataset being the most frequently used (n=\textcolor{red}{NNN}), followed by The Cancer Genome Atlas (TCGA)(n=\textcolor{red}{NNN}), Brain Tumor Segmentation Challenge (BraTS),(n=\textcolor{red}{NNN}), and Computational Precision Medicine Radiology-Pathology challenge on brain tumor classification dataset (CPM-RadPath) (n=\textcolor{red}{NNN}). Only a limited number of studies conducted external validation of their models (n=\textcolor{red}{NNN}), while the majority employed cross-validation (n=\textcolor{red}{NNN}) and internal validation (n=\textcolor{red}{NNN})

\textbf{Respiratory system (n=\textcolor{red}{NNN})}\\
Research in the respiratory system predominantly addresses diagnosis (n=\textcolor{red}{NNN}) or survival (n=\textcolor{red}{NNN}) in Covid-19 and diagnosis (n=\textcolor{red}{NNN}) or survival (n=\textcolor{red}{NNN}) of lung malignancies. For example, \textit{Lee et al.} utilized a commercially available chest X-ray abnormality detection model to extract features, which were then integrated with clinical variables and laboratory findings to predict prognostic and intervention outcomes in COVID-19 patients \cite{lee_development_2022}. \textit{Gao et al.} proposed a multimodal approach combining CT imaging and clinical variables to enhance cancer risk estimation in patients with indeterminate pulmonary nodules \cite{gao_reducing_2022}. Across these studies, the common strategy involves combining clinical variables with either X-ray or CT imaging of the thorax. Additionally, a subset of papers (n=\textcolor{red}{NNN}) developed vision-language models by integrating chest X-rays with clinical reports, specifically for X-ray report generation. Development of such vision-language models is primarily encountered in the respiratory domain probably due to the availability of the MIMIC-CXR dataset \cite{johnson_mimic-cxr_2019}. Other publicly available datasets employed by the studies of the respiratory system category are The Cancer Genome Atlas (TCGA) and the Radiological Society of North America (RSNA) dataset. Another notable observation in this anatomical subset relates to the comparatively high proportion of studies (n=\textcolor{red}{NNN}) employing external validation. Lastly, in studies comparing multimodal models against unimodal baselines, all but one demonstrated improved performance with multimodal integration.

\textbf{Reproductive system (n=\textcolor{red}{NNN})}\\
The breast domain encompasses studies focused on the diagnosis (n=\textcolor{red}{NNN}), survival prediction (n=\textcolor{red}{NNN}), and treatment response prediction (n=\textcolor{red}{NNN}) for breast malignancies. \textit{Holste et al.} evaluated various methods for fusing MRI and clinical variables in breast cancer classification \cite{holste_end--end_2021}. \textit{Wang et al.} explored multiple instance learning techniques to combine histopathology with clinical features to predict the prognosis of HER2-positive breast cancer patients \cite{wang_predicting_2023}. \textit{Joo et al.} integrated imaging features from both T1- and T2-weighted MRI along with clinical features to predict treatment response to neoadjuvant chemotherapy in breast cancer \cite{joo_multimodal_2021}. Unlike other domains, there was no predominant combination of modalities; histopathology and omics data (n=\textcolor{red}{NNN}), MRI and clinical variables (n=\textcolor{red}{NNN}), and histopathology and clinical variables (n=\textcolor{red}{NNN}) were explored with similar frequency. The use of external validation was comparable to that in the respiratory domain (\textcolor{red}{NNN}/\textcolor{red}{NNN}), which can be attributed to the availability of the TCGA-BRCA dataset employed in a high number of the studies (\textcolor{red}{NNN}/\textcolor{red}{NNN}).

\textbf{Digestive system (n=\textcolor{red}{NNN})}\\
In the domain of digestive system, most studies focused on the diagnosis of malignancies (n=\textcolor{red}{NNN}), with fewer addressing survival (n=\textcolor{red}{NNN}) and disease progression prediction (n=\textcolor{red}{NNN}). The primary malignancies investigated include colorectal (n=\textcolor{red}{NNN}) and hepatic (n=\textcolor{red}{NNN}) cancers, with some studies also focusing on the stomach (n=\textcolor{red}{NNN}) and esophagus (n=\textcolor{red}{NNN}). \textit{Guo et al.} proposed a multi-scale multiple instance learning approach to extract information from histopathology slides and integrate it with clinical variables for predicting lymph node metastasis in primary gastric cancer \cite{guo_prediction_2023}. \textit{Zhou et al.} combined histopathology slides, clinical variables, and mutation signatures for patient stratification in colon adenocarcinoma  \cite{zhou_integrative_2023}. \textit{Zhou et al.} merged PET/CT features, histopathology slides, and clinical data to predict treatment response to bevacizumab in liver metastasis originating from colorectal cancer \cite{zhou_deep_2023}. Similar to the scenario with breast studies, no single modality combination was dominant in this field, though histopathology slides (n=\textcolor{red}{NNN})/(n=\textcolor{red}{NNN}) and clinical variables (n=\textcolor{red}{NNN})/(n=\textcolor{red}{NNN}) were commonly included. The integration of multimodal data improved performance in \textcolor{red}{NNN}/\textcolor{red}{NNN} papers compared to unimodal approaches. However, external validation was relatively uncommon (n=\textcolor{red}{NNN}), proposing the need for a greater availability of public datasets. Indeed, only a few studies employed publicly available datasets including TCGA (n=\textcolor{red}{NNN}), cBIOPortal (n=\textcolor{red}{NNN}), and CPTAC (n=\textcolor{red}{NNN}).

\textbf{Sensory system (n=\textcolor{red}{NNN})}\\
In the sensory system, the majority of multimodal models have focused on ophthalmology (n=\textcolor{red}{NNN}), with the remaining studies addressing otology (n=\textcolor{red}{NNN}) and nasopharyngeal disorders (n=\textcolor{red}{NNN}). Within ophthalmology, there is a distinct focus on glaucoma (n=\textcolor{red}{NNN}) and retinopathy (n=\textcolor{red}{NNN}). For example, \textit{Mehta et al.} integrated optical coherence tomography, color fundus photography and clinical variables to diagnose glaucoma \cite{mehta_automated_2021}. \textit{Zhou et al.} employed a multimodal approach that combined four imaging modalities with free-text lesion descriptions for uncertainty-aware classification of retinal artery occlusion \cite{zhou_uncertainty-aware_2024}. \textit{Sundgaard et al.} followed an unconventional multimodal approach by integrating wideband tympanometry (a signal) with otoscopy (an image) to demonstrate that disparate data types can be effectively fused with the appropriate model architecture \cite{sundgaard_multimodal_2024}. The combination of optical coherence tomography and color fundus photography, sometimes supplemented with clinical data, was a popular approach, appearing in \textcolor{red}{NNN}/\textcolor{red}{NNN} studies. However, only a small number of papers (n=\textcolor{red}{NNN}/\textcolor{red}{NNN}) included external validation or used publicly available datasets (n=\textcolor{red}{NNN}/\textcolor{red}{NNN}).

\textbf{Integumentary system (n=\textcolor{red}{NNN})}\\
All studies within the skin category focused on the classification of skin lesions, primarily through the fusion of dermatoscopic images and clinical variables (n=\textcolor{red}{NNN})/(n=\textcolor{red}{NNN}). For example, \textit{Tang et al.} proposed two fusion schemes to efficiently integrate dermatoscopic images, clinical photographs and clinical variables for the diagnosis of eight types of skin lesions \cite{tang_fusionm4net_2022}. \textit{Zhu et al.} demonstrated that their multimodal model, which incorporated clinical images and high-frequency ultrasound, performed on par or better than dermatologists in diagnosing seventeen different skin diseases \cite{zhu_deep_2024}. Notably, all studies (n=\textcolor{red}{NNN}) comparing multimodal approaches to unimodal baselines reported improved performance with the addition of extra modalities, suggesting that factors such as lesion location and patient demographics contribute valuable information. Most studies conducted ablation analyses (n=\textcolor{red}{NNN}), demonstrating improved performance with multimodal models. Notably, one paper conducted prospective validation of its findings \cite{zhu_deep_2024}. Among the remaining studies, only one carried out external validation, while all others relied on internal validation or cross-validation approaches. In contrast to other systems, several publicly available datasets are readily accessible. The most used one is the dataset coming from the ISIC challenge (n=\textcolor{red}{NNN}), followed by HAM10000, Seven-point Criteria Evaluation (SPC), Gland Segmentation in Colon Histology Images Challenge (GlaS), and PAD-UFES-20 datasets.

\textbf{Urogenital system (n=\textcolor{red}{NNN})}\\
In the urogenital system, the majority of studies focused on the diagnosis of kidney (n=\textcolor{red}{NNN}) and prostate (n=\textcolor{red}{NNN}) disorders, with fewer addressing bladder (n=\textcolor{red}{NNN}), cervix (n=\textcolor{red}{NNN}), and ovarian (n=\textcolor{red}{NNN}) conditions. These studies predominantly involved malignancies (n=\textcolor{red}{NNN}), where multimodal models were employed for diagnosis (n=\textcolor{red}{NNN}) or survival prediction (n=\textcolor{red}{NNN}). For instance, \textit{Ning et al.} developed a comprehensive fusion method that integrated RNA sequencing, CT imaging, histopathology, and clinical variables for prognosis prediction in clear cell renal cell carcinoma \cite{ning_integrative_2020}. \textit{Priester et al.} combined MRI, prostate-specific antigen values, and prostate biopsy results to detect prostate cancer \cite{priester_prediction_2023}. A notable feature of this domain was the comparatively frequent incorporation of histopathology as modality (n=\textcolor{red}{NNN})/(n=\textcolor{red}{NNN}). Most studies (n=\textcolor{red}{NNN}) demonstrated improved performance with multimodal models compared to unimodal ones. Similarly to other systems, only a small number (2/11) externally validated their results, while the majority used either internal validation (n=\textcolor{red}{NNN}) or cross-validation (n=\textcolor{red}{NNN}) approaches. Only two studies used publicly available images coming from The Cancer Genome Atlas (TCGA) and The Cancer Imaging Archive (TCIA).

\textbf{Cardiovascular (n=\textcolor{red}{NNN})}\\
Research in the cardiovascular domain was exclusively focused on the diagnosis of heart diseases. In all but one study, the proposed models incorporated clinical variables, often in conjunction with radiology imaging (n=\textcolor{red}{NNN})/(n=\textcolor{red}{NNN}). For example, \textit{Venugopal et al.} integrated information from electronic health records, electrocardiograms and genetic data to develop a risk prediction model for cardiovascular diseases. When comparing the multimodal models to the unimodal ones, most of the studies obtained better results with the latter (n=\textcolor{red}{NNN}). However, also in this case, only two studies externally validated their results. Interestingly, some publicly available datasets were employed, including MIMIC, JSRT Database, Montgomery County X-ray Set, and data coming from the Gene Expression Omnibus (GEO) and UK Biobank.

\textbf{Miscellaneous (n=\textcolor{red}{NNN})}\\
This category includes papers that do not fit into the aforementioned categories but provide novel or unique contributions to multimodal model development. For instance, \textit{Schilcher et al.} aggregated X-ray imaging and clinical information from 72 radiology departments in Sweden to develop a multimodal model for detecting atypical femur fractures \cite{schilcher_fusion_2024}.  \textit{Lee et al.} explored unsupervised learning by combining histopathology and clinical data, followed by knowledge distillation to derive a unimodal histopathology model for predicting immunochemotherapy response \cite{lee_prediction_2024}. Additionally, \textit{Chen et al.} employed weakly-supervised learning to integrate histopathology and molecular profiles for survival outcome prediction across fourteen different cancer types \cite{chen_pan-cancer_2022}. Notably, their method incorporated a strong explainability component with heatmaps for histopathology and SHAP values for genomic markers, serving as justification for the predicted risk stratification.  

Papers still with multimodal category:

"MDF-Net for abnormality detection by fusing X-rays with clinical data" ---- MIMIC

"Medical transformer for multimodal survival prediction in intensive care: integration of imaging and non-imaging data" -- MIMIC

"Multimodal Deep Learning for Integrating Chest Radiographs and Clinical Parameters: A Case for Transformers" -- MIMIC

"Knowledge-enhanced visual-language pre-training on chest radiology images" -- MIMIC

"Deep learning algorithm-based multimodal MRI radiomics and pathomics data improve prediction of bone metastases in primary prostate cancer" -- it uses images prostate data to early predict bone metastases


"Long-term cancer survival prediction using multimodal deep learning" -- 33 types of cancers

"Deep learning with multimodal representation for pancancer prognosis prediction" -- 20 types of cancers

"Pan-cancer integrative histology-genomic analysis via multimodal deep learning" -- 14 types of cancers


"Pre-trained multilevel fuse network based on vision-conditioned reasoning and bilinear attentions for medical image visual question answering" -- in the question-answer task it is difficult to detect which organs are employed

"Caption-Aware Medical VQA via Semantic Focusing and Progressive Cross-Modality Comprehension" -- in the question-answer task it is difficult to detect which organs are employed

==> deprecated_individual_sections/medical_tasks_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Nervous system (n=95)}\\
Tasks: the majority of papers are about Alzheimer’s disease (n=36) and Cancer (glioma, glioblastoma) (n=16), other minorities include Parkinson's, Schizophrenia, Mild cognitive impairment, Epilepsy, Depression, Autism, Stroke, Mental disorders\\
Modality used: Mainly MRI with clinical data followed by MRI with omics\\
Better than unimodal: only a few studies performed an ablation study to understand the benefit of adding multiple modalities (n=28); considering these studies, in the majority of them the multimodal model reached better performances than unimodal ones (n=18) \\
External validation: only a few papers externally validated their models (n=10), the majority of papers performed cross-validation (n=49) and internal validation (n=32)\\

Brain (94)
\begin{itemize} [noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Alzheimer’s disease (36) \\
        1. Multi-modal sequence learning for Alzheimer's disease progression prediction with incomplete variable-length longitudinal data
        2. Cascaded Multi-Modal Mixing Transformers for Alzheimer's Disease Classification with Incomplete Data
    \item 	Autism (3)
    \item 	Stroke (4)
    \item 	ADHD (1)
    \item 	Cancer (16) - Glioma, Glioblastoma, cancer \\
        1.	Multi-modal Learning with Missing Data for Cancer Diagnosis Using Histopathological and Genomic Data
        2.	Augmented Radiology: Patient-Wise Feature Transfer Model for Glioma Grading
        3.	Survival Prediction of Brain Cancer with Incomplete Radiology, Pathology, Genomic, and Demographic Data
    \item 	Depression (3)
    \item 	Epilepsy (4)
    \item 	Mild Cognitive impairment (4) \\
        1.	Sociodemographic data and augmentation for MRI-based detection of amnestic mild cognitive impairment using deep learning systems
    \item 	Mental disorders (4)
    \item 	Parkinson (5)
    \item  Schizophrenia (5)
\end{itemize}

Spine (1) \\

\textbf{Respiratory system (n=60)}\\
Tasks: the majority of papers are about Covid-19 (n=23) and Tumors (adenocarcinoma, squamous cell carcinoma, non-small cell lung cancer, nodules, metastasis, malignant pleural mesothelioma) (n=21), other minorities include Chronic Obstructive Pulmonary Disease, Pneumonia, Embolism, Tuberculosis, other pulmonary diseases\\
Modality used: Mainly CT and clinical variables, followed by X-ray with clinical variables\\
Better than unimodal: most of the studies performed an ablation study to understand the benefit of adding multiple modalities (n=43) of which all studies except one obtained better results with their multimodal model\\
External validation: 10 external, 18 internal cross-validation, 28 internal validation\\
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Lung cancer (21) \\
        i.	Reducing uncertainty in cancer risk estimation for patients with indeterminate pulmonary nodules using an integrated deep learning model
        ii.	Deep Multi-path Network Integrating Incomplete Biomarker and Chest CT Data for Evaluating Lung Cancer Risk
        iii.	Multi-modality Fusion Based Lung Cancer Survival Analysis with Self-supervised Whole Slide Image Representation Learning
        iv.	Deep-learning-enabled multimodal data fusion for lung disease classification
    \item	Covid-19 (23) \\
        i.	Multimodal graph attention network for COVID-19 outcome prediction
        ii.	Development and Validation of a Multimodal-Based Prognosis and Intervention Prediction Model for COVID-19 Patients in a Multicenter Cohort
    \item	Other pulmonary disease \\
\end{itemize}

\textbf{Gastrointestinal (n=27)}\\
Tasks: the majority of papers are about cancer (colorectal, gastric, hepatocellular cancers), other diseases include pancreatitis, dental caries, enterocolitis, fibrosis\\
Modality used: several different combinations of modalities are present, there is no predominant combination, 12/27 used pathology, 15/27 used clinical variables, only 2 used unstructured text, and only 4 used omics\\
Better than unimodal: most of them performed ablation studies (n=21) and only in one of these studies the multimodal model was not better than the unimodal one.\\
External validation: most papers employed a cross-validation (n=12) or internal validation (n=10) strategy, only a few externally validated the results (n=4)\\
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Colorectal (6)
    \item Liver (7)
    \item Stomach (2)
    \item Esophagus (2)
    \item Duodenum (1)
    \item Gastrointestinal (3)
    \item Mouth (1), oral tract (3) 
    \item Pancreas (1)\\
\end{itemize}

\textbf{Breast (29)}
Tasks: all cancer related\\
Modality used: no predominant modality combinations are present, pathology and omics with or without a third modality (n=4), pathology and clinical variables (n=4), MRI and clinical variables (n=5)\\
Better than unimodal: most of them performed ablation studies (n=24), and the majority resulted in better performances using the multimodal model (n=23) \\
External validation: most papers employed an internal validation (n=15) strategy, and only a few externally validated the results (n=6), and some others just internally validated (n=6)\\
Predicting the prognosis of HER2-positive breast cancer patients by fusing pathological whole slide images and clinical features using multiple instance learning\\

\textbf{Sensory (n=27)}
Tasks: mainly eyes (n=24), some studies about ear. Cancer (lymphoma 1, glaucoma 9), retinopathy (4), cardiovascular disease (3), other diseases (occlusion 1, atrophy 1, …)\\
Modality used: fundus and OCT, alone or with a third modality, are the most used combination for eye studies (n=9), then fundus and clinical variables (n=4), in the majority of the combinations, clinical variables are added to another modality (n=14)\\
Better than unimodal: 18/19 studies that performed ablation analysis reached better performances with the multimodal model \\
External validation: only 2 externally validated the results, 13 internally validated, and 12 cross-validated\\
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Eyes (n=24) \\
        i. Uncertainty-aware incomplete multimodal fusion for few-shot Central Retinal Artery Occlusion classification
    \item Ear (n=2)
    \item Nasopharynx (n=1)\\
\end{itemize}

\textbf{Skin (18)}
Tasks: All of them performed skin lesion classification, the majority of them classified cyst, nevus, and keratosis from different types of carcinoma, i.e., basal cell carcinoma, squamous cell carcinoma, melanoma.\\
Modality used: mostly dermatoscopic images with clinical variables (n=13), few studies used ultrasound images (n=2), only one used pathology and clinical variables, one used unstructured text with dermatoscopy images\\
Better than unimodal: all studies that performed an ablation study resulted in better performances with the multimodal model (n=12)\\
External validation: only 1 externally validated the results, 12 internally validated, and 3 cross-validated, 1 prospective validation (the reviewer was not sure about this)\\

\textbf{Urogenital (n=14)}
Tasks: The majority focused on kidney (n=7), a few on prostate (n=4), bladder, cervix and ovary. They focus on diagnosis (n=6) and survival prediction (n=5) of cancer patients (n=11) and diagnosis of other diseases, e.g., renal artery stenosis (n=1), chronic kidney disease (n=1), and renal report generation (n=1)\\
Modality used: most of them combined pathology with another modality (n=9), between omics, clinical variables, and radiology\\
Better than unimodal: 8/11 obtained better results with their multimodal model\\
External validation: only 2 externally validated the results, 7 internally validated, and 5 cross-validated \\
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Prostate (n=4) 
    \item Prostate cancer therapy personalization via multi-modal deep learning on randomized phase III clinical trials
    \item Kidney (n=7) \\
        i.	MPCITL: design of an efficient multimodal engine for Pre-emptive identification of CKD via incremental transfer learning on clinical data samples
        ii.	Integrative analysis of cross-modal features for the prognosis prediction of clear cell renal cell carcinoma
    \item Bladder (n=1)
    \item Cervix (n=1)
    \item Ovary (n=1)\\
\end{itemize}

\textbf{Cardiovascular (n=13)}
Tasks: The majority focused on the diagnosis of heart diseases (n=11), such as cardiomegaly, cardiovascular risk, coronary artery disease, cardiomyopathy, myocardial infarction, pulmonary venous obstruction, ischemic disease, embolism, only a few focused on survival prediction (n=2) of ICU or ischemic patients.\\
Modality used: all studies except one combined clinical variables with another modality, omics (1), radiology (7), pathology (1), unstructured text (1), signal+omics (1), other (1). One study combined signals and X-ray.\\
Better than unimodal: 10/11 obtained better results with their multimodal model (one obtained almost the same results with unimodal, slightly better with multimodal but non significantly better)\\
External validation: 2 external, 4 internal validation and 7 internal cross-validation\\
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Heart (13)\\
        i.	A novel attention-based cross-modal transfer learning framework for predicting cardiovascular disease	
    \item Blood (1)  \\
\end{itemize}

\textbf{Musculoskeletal (5)}
Tasks: Diagnosis of fractures, bone aging, osteoarthritis (n=2) and Prosthetic Joint Infections\\
Modality used: X-ray combined with unstructured text (n=1), clinical variables (n=2) and clinical variables+MRI (n=1). One study on CT and unstructured text.\\
Better than unimodal: 3 ablation study where the multimodal model performed better than unimodal ones\\
External validation: 4 internal validation and 1 cross-validation\\

Fusion of electronic health records and radiographic images for a multimodal deep learning prediction model of atypical femur fractures

==> deprecated_individual_sections/missing_data_handling.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Missing data handling} \label{sssec:Missing data handling}

Most multimodal AI models work on the assumption of data completeness, meaning that all required modalities are available for every entry. However, this is often not feasible due to issues such as privacy and device limitations or missing data due to the study's retrospective nature. Handling missing data without introducing bias into the analysis presents a significant challenge. Indeed, a commonly employed approach to address this issue is to exclude all entries with at least one missing modality and include only complete entries in the dataset used for analysis, and this is the case for \textcolor{red}{79\% (212/268)} of the included papers. Although the exclusion of incomplete entries is a quick and straightforward method for handling missing data, this approach results not only in decreasing the data sample size and potentially losing useful information contained in the discarded samples but also limits the model inference to complete-modality data and inevitably leads to selection biases, thereby potentially compromising the validity and generalizability of the analysis. Rather than discarding incomplete samples, missing information can be estimated using imputation techniques. These techniques can be broadly divided into two categories: non-learning-based and learning-based approaches. \\

\textbf{Non-learning-based approaches} \\ The findings of our study indicate that the first category is predominantly utilized, with 52\% (29 out of 56) of the reviewed studies implementing non-learning-based techniques. These techniques are primarily employed to impute values of structured data (20 out of 29 studies \textcolor{red}{references}), such as clinical variables and test results. Less frequently, these methods are used to address missing gene values (3 out of 29 studies \textcolor{red}{references}) or image modalities (1 out of 29 studies \textcolor{red}{references}). For continuous variables, imputation is performed using measures of central tendency such as the mean or median. For categorical variables, imputation strategies include using the most frequent category (mode) or introducing a new category for missing values. Other studies (3/29 \textcolor{red}{references}) employed the Multivariate Imputation by Chained Equations (MICE) algorithm. This method uses multiple imputation techniques to fill in the missing data and then combines the results from multiple imputations to produce a final imputed dataset \textcolor{red}{references}. Additionally, some papers used fixed values to handle missing data, including zero imputation, where missing values are replaced with zeros \textcolor{red}{references}, a modified version of this approach where missing values are replaced with -1 \textcolor{red}{references}, or the hot-deck method, which involves replacing missing values with randomly selected values from similar records \textcolor{red}{references}. Other statistical methods include the moving average, which replaces missing values with the average of a specified number of surrounding data points and uses a linear regression trained on the complete data to predict the missing ones \textcolor{red}{references}. The fixed-value imputation methods are straightforward and often used for their simplicity and ease of implementation. However, they, along with statistical methods, can introduce bias and reduce variability in the data. \\

\textbf{Learning-based approaches} \\ Some studies utilized machine learning methods to predict missing values based on patterns learned from complete data, offering an alternative to simpler imputation techniques. Among machine learning methods, studies employed the k-nearest neighbor (k-NN) method, which imputes missing values based on the values of the nearest neighbors in the feature space \textcolor{red}{references}, and the weighted nearest neighbor approach \textcolor{red}{references}, which assigns weights to neighbors based on their distance, giving more influence to closer neighbors in the imputation process. Other studies \textcolor{red}{references} employed the Classification and Regression Trees (CART) algorithm, which utilizes decision trees to predict missing values by partitioning the data into homogenous subsets, while another study \textcolor{red}{references} employed the XGBoost that is capable of learning the branch directions of the trees for missing variables directly during training. \\
 More sophisticated methods involve the application of deep learning models to impute missing values, and the management of an arbitrary number of modalities directly modifying the model architecture to process incomplete data without imputation. 
Some examples of imputing missing modalities through deep learning models are \cite{xu_explainable_2022} which employed a Dynamic Multimodal Variational Autoencoder, utilizing a product-of-experts structure to infer missing modality features based on existing data, \cite{dolci_deep_2023} which employed Generative Adversarial Networks (GANs) to generate missing domain data, e.g., from neuroimaging data to genomics data, or vice versa, and \cite{saad_learning-based_2022} which utilized a deep convolutional neural network to generate synthetic miRNA data from PET scans to compensate for missing miRNA information. Finally, \cite{xu_multi-modal_2022} proposed a multimodal sequence learning framework that uses a deep latent representation collaborated sequence learning strategy. This framework includes a deep multimodality fusion module, including degradation networks that capture complementary information from incomplete multimodal data, which are then used in a sequence learning module to model Alzheimer's disease progression.

Some papers have addressed the challenge of missing data by designing specific loss functions that account for incomplete modalities. For instance, \cite{gao_deep_2021} employed a cross-entropy loss across three distinct paths—image-path, biomarker-path, and combined path—allowing the model to train only on the available modalities. Similarly, \cite{taleb_contig_2022} used a contrastive loss with an inner aggregation scheme for complete datasets and an outer scheme that handles incomplete instances by calculating distances based on the present modalities. \cite{cui_multi-modal_2022} introduced a structured hidden representation that integrates available modality features, using reconstruction and classification losses to maintain a common space for comparing samples with varying modalities. Furthermore, \cite{kawahara_seven-point_2019} defined a multimodal multi-task loss function, summing several losses that each depend on different combinations of input modalities, enabling the model to make predictions based on the available data during inference. Finally, \cite{cui_survival_2022} employed a modality dropout to boost fusion capabilities with missing data, fusing the modalities by averaging the available modality embeddings. To encourage the model to learn cross-modality information, they introduced a reconstruction loss to ask the model to reconstruct the intentionally dropped-out modality. 

Some other studies have leveraged transformer architectures to address the challenge of incomplete data without relying on imputation. For instance, \cite{liu_cascaded_2023} introduced a Cascaded Modality Transformer, which uses a sequence of transformer decoder blocks where each block processes the output from the previous modality transformer. To simulate missing data, a Modality Dropout module randomly zeros out specific modalities with a probability P. Similarly, \cite{zhou_uncertainty-aware_2024} utilized a transformer capable of handling input sequences of arbitrary lengths, allowing the model to manage cases with missing or incomplete modalities effectively. In another example, \cite{khader_multimodal_2023} trained a transformer on complete data and then evaluated its performance with patient data from the test set, where some input parameters were randomly omitted. This approach mimics human reasoning, with the model’s performance gradually declining as more clinically relevant data is missing. 



\begin{itemize}
    \item seems that \citet{dolci_deep_2022} is of almost the same authors of \citet{dolci_deep_2023}, they are both conference proceedings on the same topic/task. To exclude the older one?
    \item \citet{akramifard_early_2021} not clear

\end{itemize}



==> deprecated_individual_sections/overview.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Review of the state of the art in multimodal medical AI}\label{overview_modalities}
The landscape of multimodal artificial intelligence (AI) in medical research has expanded between 2018 and 2024, as shown by the growing number of articles focused on integrating multiple modalities. Subdividing the 331 articles in this review per year (Figure 1(A)), we see a rapid increase, starting with 3 papers in 2018 to 109 papers in 2023. 

We distributed the reviewed papers according to data modalities, which will be broadly described here. Subsequently, the review is organized according to the following subsections:

\begin{itemize}
    \item State-of-the-art algorithm design for multi-modal medical AI (section \ref{sssec:architecture choices})
    \item Clinical tasks (section \ref{sssec:Clinical applications}) for a detailed analysis of the multimodal AI approaches categorized per organ system
    \item Challenges and opportunities for clinical adoption (section \ref{ssec:road_to_the_clinic} for selected examples of multimodal AI in clinical practices.
\end{itemize}

Last, we will discuss our findings and provide guidelines for future research directions.

\subsection{Summary of multimodal medical AI research} \label{sssec:Current landscape of multimodal AI in medical research}

\textbf{Modalities in medical AI research}\\
We divided the data modalities into image-based and non-image-based modalities. The image-based modalities are grouped according to their related medical specialties. If there were too few papers for a medical specialty, we grouped them into a catch-all 'other' category, namely radiology (computed tomography (CT), magnetic resonance imaging (MRI), ultrasound (US), X-rays, and nuclear imaging (SPECT/PET)), pathology (stained histology images) and other (includes optical coherence tomography (OCT), fundus photography and dermatoscopy). Meanwhile, the non-image-based modalities consist of texts (structured texts such as test result tables and unstructured texts such as medical reports), 'omics data (e.g., genomics, transcriptomics, or proteomics), and other non-image modalities (such as EEG or ECG). \\

Among the 331 reviewed papers, 10 stood out for focusing on multiple medical tasks or their application in multiple diseases. The papers were categorized based on the types of data modalities they used. The largest of these studies (about 30\% each) focused on radiology and text-based data. Pathology and 'omics data each comprised of 11\% and 10\% of the studies, respectively. The remaining studies were categorized into "other image-based modalities" (7\%) and "Other non-image-based modalities" (9\%). Figure 1(B) visualizes these data modality groups and their respective subtypes. \\

\textbf{Commonly used combinations}\\
The analysis of modality combinations in the studied multimodal AI papers reveals interesting patterns (see Figure 1(D)). The most prevalent combination is radiology with text (141 studies), followed by 'other' - text (27), pathology - 'omics (25), text - other non-image modalities (24) and radiology-omics (21). These top combinations highlight the trends in integrating visual data with tabular or text data. Interestingly, while the radiology-pathology combination appears frequently in conjunction with other modalities, it is less common as a standalone pair (10), suggesting that studies often find values in integrating this visual modality pair with additional data types. \\

The review also reveals several complex combinations involving three or more modalities, albeit in smaller numbers. Notably, radiology-omics-texts (11) pathology-omics-texts (10), and radiology-pathology-omics-texts (3) demonstrate the attempts to create comprehensive models that span multiple scales of biological organization - from organ-level (radiology) to tissue and cellular (pathology) and subcellular (omics), complemented by clinical contexts (texts). \\


\subsection{Key application areas} \label{sssec:Key application areas}
Eleven medical disciplines were identified from the studied papers (see Figure 2 for the complete list). Among the medical disciplines, the nervous system dominates with 96 studies, followed by respiratory (63), breast (29), and gastrointestinal (28) systems. A substantial number of studies (42) fall under the miscellaneous category, which is further explained in the dedicated section Medical tasks (section \ref{sssec:Medical tasks}). \\

We divided the medical tasks into diagnosis, prognosis, and treatment. In prognosis studies, we further sub-categorized them into survival, disease progression, and treatment response. Studies without a clear medical task were listed as "not applicable". In terms of medical tasks, diagnosis emerged as the primary focus across all disciplines, accounting for 52-73\% of each medical discipline. Survival analysis followed as the second most common task (7-9\%). Other prognostic tasks, such as prediction of disease progression or treatment response, were not uniformly represented across all disciplines. \\

We divided the AI tasks into classification (for categorical prediction), regression (for continuous values prediction), image or signal detection or segmentation, and text generation. The strong correlation between most medical tasks and classification AI tasks (e.g., diagnosis at 0.86, disease progression at 0.75, and treatment response at 0.93) demonstrates the current emphasis on categorical predictions in multimodal AI medical applications. The analysis also revealed some notable gaps and opportunities in the field. For example, the few studies focused on treatment (only 1 study), and the limited representation of detection, segmentation, and text generation AI tasks resulted in poor correlation with medical tasks. These findings suggest potential technical limitations imposed by the data modalities and the available sources of shared multimodal datasets, which will be discussed in the following.\\


\onecolumn
\begin{figure}%
    \centering
    \includegraphics[width=15cm]{figures/fig_distribution_of_modalities.png}%
    \caption{(A) Distribution of studies by year. Bar chart shows the number of studies per year from 2018 to 2024. (B) Pie chart shows the proportions of different modality groups and the respective data modalities used across studies. (C) Bubble chart shows the distribution of data modalities over the year from 2018 to 2024. (D) Diagram shows connections between modalities. (Daan and Geert: add extrapolation for another 5 years) (TODO: Change prediction to regression; otherimage to Clinical images)\\}% 
    \label{fig:fig_distribution_of_modalities}%
\end{figure}


\begin{figure}%
    \centering
    \includegraphics[width=20cm]{figures/fig_distribution_medical_disciplines_tasks.png}%
    \caption{Medical disciplines, medical tasks and AI tasks}%
    \label{fig:fig_distribution_medical_disciplines_tasks}%
\end{figure}

\begin{figure}%
    \centering
    \includegraphics[width=18cm]{figures/fig_distribution_of_encoder_fusion_modality.png}%
    \caption{Distribution of encoder and fusion methods, and their respective correlations with data modalities}%
    \label{fig:fig_distribution_of_encoder_fusion_modality}%
\end{figure}


\begin{figure}%
    \centering
    \includegraphics[width=18cm]{figures/fig_distribution_of_public_datasets.png}%
    \caption{Public datasets used across all reviewed papers, and the trend of these public datasets usage over the years. (TODO: remove Publication data and mention it in the text)}%
    \label{fig:fig_distribution_of_public_datasets}%
\end{figure}



\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|p{2cm}|p{10cm}|p{1cm}|p{1cm}|}
        Ref & \textbf{Databases or public dataset sources} & Link & \textbf{Count} \\
        \hline
         & Publication & & 161 \\
         & The Cancer Genome Atlas (TCGA) &  & 49 \\
         & Alzheimer's Disease Neuroimaging Initiative (ADNI) &  & 38 \\
         & Medical Information Mart for Intensive Care (MIMIC) & 	& 22 \\
         & Computational Precision Medicine Radiology-Pathology challenge on brain tumor        classification (CPM-RadPath) &  & 7 \\
         & The Cancer Imaging Archive (TCIA) &  & 6 \\
         & Kaggle &  & 6\\
         & International Skin Imaging Collaboration (ISIC) &  & 5 \\
         & GLAS &  & 4 \\
         & MoNuSeg &  & 4 \\
         & Parkinson's Progression Markers Initiative (PPMI) &  & 4 \\
         & Autism Brain Imaging Data Exchange (ABIDE) &  & 4 \\
         & National Lung Screening Trial (NLST) &  & 3 \\
         & PadChest &  & 3 \\
         & MFFD &  & 3 \\
         & DAIC-WOZ &  &  3 \\
         & QaTa-COV19 &  & 3 \\
         & HAM10000 &  & 3 \\
         & Radiological Society of North America (RSNA) &  & 3 \\
         & CoSKEL &  & 3 \\
         & UK Biobank (UKB) &  & 2 \\
         & Brain Tumor Segmentation Challenge (BraTS) &  & 2 \\
         & National Institute of Health (NIH) &  & 2 \\
         & Osteoarthritis Initiative (OAI) &  & 2 \\
         & Github &  & 2 \\
         & METABRIC &  & 2 \\
         & Open Access Series of Imaging Studies (OASIS) &  & 2 \\
         & cBioPortal &  & 2 \\
         & ISIC 2018 Challenge &  & 2 \\
         & The Australian Imaging Biomarker \& Lifestyle Flagship Study of Ageing (AIBL) &  & 2 \\
         & CPTAC &  & 2 \\
         & National Alzheimer's Coordinating Center (NACC) &  & 2 \\
         & PAD-UFES-20 &  & 2 \\
         & Brain Tumor Segmentation Challenge (BraTs) &  & 2 \\
         & CheXpert &  & 2 \\
    \end{tabular}}
    \caption{List of public databases and the use of public datasets. (TODO: Add links and references)}
    \label{tab:List of public databases and the use of public datasets}
\end{table}

\twocolumn
\subsection{Methodological approaches} \label{sssec:Methodological approaches}
\textbf{Data sharing in the studies}\\
The utilization of public datasets in multimodal AI research for medical applications is widespread, with 84\% (287 out of 332) of the reviewed papers incorporating such resources in their model development and validation processes. Among these studies, the majority (192 papers) relied on a single dataset source, while other studies integrated data from multiple sources, with one study incorporating up to 21 different sources (paper ID 133). The landscape of public datasets is diverse, with the most frequent source being shared datasets from publications (161 retrievals), followed by established databases such as The Cancer Genome Atlas (TCGA, 49 retrievals), Alzheimer's Disease Neuroimaging Initiative (ADNI, 38), and Medical Information Mart for Intensive Care (MIMIC, 22). Other notable sources include the CPM-RadPath challenge (7), The Cancer Imaging Archive (TCIA, 6), and Kaggle (6), with numerous other databases being utilized in five or fewer studies. See Table \ref{tab:List of public databases and the use of public datasets}.\\ 

The impact of public datasets varies across medical disciplines, with studies focusing on the nervous system and respiratory conditions benefiting the most from these resources. ADNI, TCGA, and shared datasets from publications emerge as the primary data sources within these two fields. In contrast, research in musculoskeletal and sensory domains shows the least utilization of shared datasets. Interestingly, while most public databases are tailored to specific medical domains or disease groups, TCGA stands out as a more versatile resource. Referring to Figure \ref{fig:fig_distribution_of_public_datasets}, a temporal analysis reveals an increasing trend in the use of shared datasets from publications, as well as growing reliance on major databases such as ADNI, MIMIC, and TCGA over the years. This trend signifies the growing importance of data sharing and standardization in advancing multimodal AI research in medicine.\\


\textbf{Common data encoder and fusion techniques used}\\
Various encoder mechanisms and fusion strategies are employed to process and integrate different data modalities. Encoders are categorized into Convolutional Neural Networks (CNNs), Vision Transformers (ViTs), Recurrent Neural Networks (RNNs), Transformers, handcrafted feature encoders, multi-layer perceptrons (MLPs), multiple encoders, and others. Fusion stages, which determine when different data modalities are combined, are categorized as Early (data-level fusion), Intermediate (feature-level fusion), Late (decision-level fusion), Multiple (combination of two fusion stages), or All (incorporating early, intermediate and late fusion).\\

Summarized in Figure \ref{fig:fig_distribution_of_encoder_fusion_modality}, the analysis reveals that CNNs dominate the encoder landscape (55\% of the studies), followed by Other mechanisms (16\%) and MLPs (11\%). Notably, 1\% of the studies employed multiple encoder types. CNNs show strong correlations with image-based data modalities, including Clinical images (0.98), Radiology (0.82) and Pathology (0.77). In contrast, non-image modalities such as Omics, Texts and Other Non-image data use a more diverse range of encoders, including MLPs, traditional Machine Learning encoders, RNNs and Transformers. Regarding fusion strategies, Intermediate fusion is the most prevalent among all strategies, used in 78\% of the studies, followed by Late fusion (15\%) and Early fusion (6\%). Intermediate fusion shows strong correlations (0.65-0.91) across all modalities, while Early and Late fusion strategies exhibit weak correlations (0.02-0.22), and other fusion mechanisms were rarely used. 

% \begin{table}[ht]
%     \centering
%     \begin{tabular}{lccc}
%         \textbf{Medical tasks} & \textbf{AI tasks} & \textbf{Multimodal AI} & \textbf{Frequency} \\
%         \hline
%         Diagnosis & Classification & & 112 \\
%         & Prediction & & 8 \\
%         & Image detection & & 2 \\ 
%         & Image segmentation & & 14 \\
%         & Text generation & & 3 \\
%         \hline
%         Survival analysis & Classification & & 15 \\
%           & Prediction & & 17 \\
%           & Image segmentation & & 3 \\
%         \hline
%         Disease progression & Classification & & 12 \\
%           & Image segmentation & & 2 \\
%         \hline
%         Treatment response & Classification & & 4  \\
%         \hline
%         Not specified & Classification & & 28 \\
%           & Prediction & & 4 \\
%           & Image segmentation & & 12 \\

%     \end{tabular}
%     \caption{Distribution of tasks}
%     \label{tab:Distribution of tasks}
% \end{table}





\
%minutes
%\begin{itemize}
%    \item definitions of medical tasks, ai tasks
%    \item why do we split the tasks
%    \item forming broken bridges is okay
%\end{itemize}





==> deprecated_individual_sections/road_to_the_clinic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The road to the clinic} \label{ssec:road_to_the_clinic}
In addition to reviewing the landscape of multimodal AI models in research, we investigated to what extent these potential performance boosts can be achieved by clinicians today. To this end, we searched the \href{https://www.fda.gov/medical-devices/software-medical-device-samd/artificial-intelligence-and-machine-learning-aiml-enabled-medical-devices}{FDA database of AI/ML-enabled medical devices} and the \href{https://healthairegister.com/}{Health AI register} for multimodal AI models that obtained either FDA- or CE-clearance. Since these databases contain 950 and 213 entries, respectively, we performed an automated preselection of models that may incorporate multiple modalities. Specifically, for each entry in the FDA database, we automatically retrieved the publicly available 510(k) premarket notification summary and searched for any mention of "multi-modal" or "multimodal". This resulted in 38 hits, which were all manually inspected for the same inclusion criteria as used in the literature search. Although one product was found to fit the multimodality criterion by incorporating EEG, neurocognitive test scores and clinical symptoms to assess the need for CT imaging after potential structural brain injury \citep{hanley_emergency_2017}, no deep neural networks were involved which would place this out of scope for the current review. 

A similar strategy was employed for entries in the Health AI register, where a published  validation study, when available, was retrieved and scanned for occurrences of the word "multimodal" or "multi-modal". Although a validation study could be retrieved for 132/213 products, none of these studies returned a hit for our multimodal keywords. Combining our findings for both the Food and Drug Administration (FDA) database and AI health register, it appears that the promising multimodal AI models showcased in this review have yet to make their way to the clinic.   

However, despite the lack of FDA- or CE-certified multimodal AI models, we identified two papers during our literature search that demonstrated potential in transitioning multimodal AI models from research to clinical practice.
First, \citet{esteva_prostate_2022} describe a multimodal model that integrates digital pathology slides and clinical variables for risk stratification in prostate cancer \citep{esteva_prostate_2022}. Specifically, the model employs a ResNet50 pretrained in a self-supervised manner to extract a feature vector from the pathology slides and subsequently concatenates this image feature vector with a clinical variable vector for the final prediction. Compared to the unimodal imaging model, the multimodal obtained a notably higher AUC of 0.837 vs. 0.779 for predicting distant metastasis after 5 years. In addition, this model was externally validated in a phase 3 trial (NRG/RTOG 9902) and demonstrated significant and independent association with prognostic factors compared to current methods such as the National Comprehensive Cancer Network (NCCN) high-risk features \citep{ross_external_2024}. Given this favorable head-to-head performance comparison with current clinical prognostic methods, it has since been incorporated in the NCCN guidelines. Although this model is not FDA-certified, clinicians in the United States of America can order it as part of the regular prognostic workup of their patients. \newline
Second, \citet{lee_development_2022} focussed on the development and validation of a multimodal model for prognosis and treatment selection in COVID-19 patients \citep{lee_development_2022}. This multimodal model employed a previously validated and CE-approved chest X-ray abnormality detection model \citep{nam_development_2021} to infer imaging features from chest X-rays and fused this with clinical and laboratory data to predict prognosis and required interventions for patients with COVID-19. Retrospective validation on 2282 COVID-19 patients from 13 medical centers demonstrated that the multimodal model significantly outperformed the unimodal imaging model with an AUROC of 0.854 vs. 0.770, respectively. A feature importance analysis revealed that, among others, clinical variables such as age and dyspnea played an important role in the multimodal model's prediction. Although the multimodal itself is not available for clinicians today, this study provided evidence that current unimodal AI models can be incorporated in a multimodal model pipeline to improve their performance. \newline
\newline
To advance the translation of multimodal AI research into commercially available products, it is crucial to focus on several key strategies. Setting aside the many technical challenges inherent in multimodal AI, it is important to develop features such as multimodal learning frameworks that can learn from different data types without needing separate encoder architectures \citep{acosta_multimodal_2022}. While these specific technical aspects won't be discussed here, they are vital for streamlining the AI development process and enhancing its practical application. \newline
Firstly, the collection, curation, and harmonization of well-phenotyped, diverse, and comprehensive annotated datasets that represent various demographic factors are essential \citep{acosta_multimodal_2022}. The richness and quality of such data are paramount for training effective AI models, as they ensure robustness, generalizability, and accuracy in real-world applications. This process, however, faces challenges such as high costs associated with deep phenotyping and longitudinal follow-up, which escalate with larger participant numbers, making automated data collection methods necessary to remain financially sustainable \citep{acosta_multimodal_2022}. Another systematic problem in current multimodal datasets is the high proportion of missing data. Incomplete data can lead to selection bias, where the remaining data is not representative of the broader patient population \citep{haneuse_assessing_2021}.The likelihood of certain measurements being recorded in a patient's EHR is influenced by various factors, including diagnostic hypotheses and family medical history. This highlights the potential for selection bias to arise in the data collection process \citep{haneuse_assessing_2021}. Lastly, previous studies have demonstrated that by utilizing only a little background information about participants, an adversary could re-identify those in large datasets \citep{narayanan_robust_2008}. As the amount of multimodal data collected per patient increases, including hospital admission dates, age, photographs for skin malignancy detection, phenotyping accuracy improves, and significant privacy concerns rise, as the richer data can lead to the re-identification of individuals within large datasets. Managing these privacy issues is crucial to protect patient confidentiality while benefiting from the enhanced insights provided by comprehensive multimodal data. \newline
Secondly, the development of explainable AI (XAI) is of high importance to address the limitations of AI's "black box" nature \citep{pahud_de_mortanges_orchestrating_2024}. Explainable AI ensures that end-users can understand and trust the AI's decision-making process, which is crucial for the widespread adoption and usability of these technologies in clinical practice \citep{kline_multimodal_2022}. Prioritizing these strategies will help bridge the gap between research and practical, commercially available multimodal AI solutions in healthcare.

==> deprecated_individual_sections/search.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT EDIT THESE FILES ANYMORE, ALL CHANGES SHOULD BE DONE IN %%
%% THE main.tex FILE!!!                                           %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Search Criteria} \label{ssec:Search}

This scoping review aimed to evaluate the application of multimodal AI models in the medical field, where we define multimodality as data originating from different medical specialties. For instance, we consider a multimodal model that integrates a diagnostic CT scan and subsequent tissue biopsy slides as it combines the domains of the radiologist and the pathologist, respectively. Conversely, a model integrating T1- and T2-weighted MRI scans would not be considered multimodal. In addition to this multimodality criterion, we limited our scope to I) studies using deep neural networks and II) studies developing multimodal models for specific medical tasks (i.e., no generic visual question answering).

The literature search was conducted in PubMed, Web of Science, Cochrane, and Embase. The entire search string per database can be found in \ref{sec:appendixA}. The search was initially performed on April 16, 2024 and repeated on October 2, 2024 to ensure an up-to-date overview, yielding a total of 10,750 initial results. These results included both journal and conference papers. In addition to the previously mentioned inclusion criteria, we applied additional standard exclusion criteria summarized in figure \ref{fig:screening}. Specifically, we excluded review articles, non-English publications, articles without full text, non peer-reviewed preprints, and those published before 2018. After filtering with these criteria and deduplicating results using the DedupEndNote tool \citep{Lobbestael2023}, 9,002 articles were imported into the paper screening software Rayyan \citep{Ouzzani2016}. An additional 59 duplicates were manually removed, resulting in 8,943 articles for the Title and Abstract (TiAb) screening phase.
A team of six reviewers conducted the TiAb screening phase. Each paper's title and abstract were reviewed based on the inclusion criteria. Included papers were verified by a second reviewer and potential discrepancies were resolved through discussion or involving a third reviewer if necessary. The TiAb screening phase was performed sequentially, starting with verifying that the paper is in the medical domain, then determining whether it is in scope, whether multimodality is involved, and finally, assessing whether deep neural networks are used. Papers were deemed to be outside the scope of this review when they investigated tasks that do not have an explicit clinical question (i.e., image denoising, registration). The TiAb screening resulted in 552 articles being considered for full-text screening.

In the full-text reading phase, a single reviewer read each article in full to confirm adherence to our inclusion criteria. In case of doubt, a second reviewer was involved to arrive at a consensus decision. Eventually, 368 studies were included in the final analysis.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/multimodal_search.png}
    \caption{Overview of the screening process.}
    \label{fig:screening}
\end{figure}


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
